Oscillator-based Ising Machine

Many combinatorial optimization problems can be mapped to finding the ground states of the corresponding Ising Hamiltonians. The physical systems that can solve optimization problems in this way, namely Ising machines, have been attracting more and more attention recently. Our work shows that Ising machines can be realized using almost any nonlinear self-sustaining oscillators with logic values encoded in their phases. Many types of such oscillators are readily available for large-scale integration, with potentials in high-speed and low-power operation. In this paper, we describe the operation and mechanism of oscillator-based Ising machines. The feasibility of our scheme is demonstrated through several examples in simulation and hardware, among which a simulation study reports average solutions exceeding those from state-of-art Ising machines on a benchmark combinatorial optimization problem of size 2000.

==> PPV.tex <==
\section{Phase-macromodels and Ising Hamiltonian}\seclabel{PPV}

In this section, we concretize the mechanism of oscillator-based Ising machine
by studying oscillators’ phase macromodels and explaining why they minimize the
Ising Hamiltonian.

A single oscillator can be written as a DAE. x\_s, alpha, what is PPV.

Based on PPV, when the input is periodic, a simplified approximation has been
developed, GAE. It governs… can be used to predict IL effectively.

Note that a special case of GAE is the Adler’s equation. It captures the phase
dynamics of an oscillator with sinusoidal PPV under sinusoidal perturbation
close to the oscillator’s natural frequency. In comparison, GAE is more
generally applicable to virtually any nonlinear oscillator under any periodic
perturbation, including the case where perturbation is close to the harmonics
of the oscillator’s natural waveform.

GAE can be used to predict SHIL effectively []. Figure… LHS, RHS.

Furthermore, GAE analysis can also be applied when both SYNC and first-order
perturbation are present. Figure … plot the LHS and RHS of GAE with a fixed
SYNC and different strengths of first-order perturbation. From it we can see
how the stability of the two solutions in Fig .. change — one vanishes as D
increases, leaving only one stable solution. If D comes from another oscillator
with the same natural frequency, the stable solution indicates that the two
oscs synchronize with a phase difference.

GAE can be generalized to capture the phases of coupled oscillators []. If we
assume sinusoidal PPVs for D, we arrive at a commonly used special case of
coupled oscillator GAE model, known as the Kuramoto model:

Kuramoto model is a gradient system []. We can consider the following Lyapunov
function as its ``energy’’:

such that

dE/dt

Therefore, the coupled oscillator system always attempts to minimize the energy
E.

E as defined in () shares some similarities with the Ising Hamiltonian in ().
If all the phases of oscillators settle to binary phases 0 and pi,
corresponding to sigma equal to 1 and -1, cos(phi\_i-phi\_j) = sigma\_i *
sigma\_j. Then the coupled oscillators are naturally minimizing the Ising
Hamiltonian defined in (). In fact, this is also the mechanism with which many
other coupled oscillator schemes work for pattern recognition, image
segmentation, etc.

It is trivial to prove that two coupled oscillators will settle with phase
difference of either 0 or pi, depending on the polarity of J\_12. However, as
the number of oscillators increases, the phases may not settle to binary
values. In other words, the system becomes more and more an analog computer
than a digital combinatorial optimizer. As we discuss in Sec …, one intuition
behind oscillator-based Ising machines is that an oscillator behaves like a
binary latch. To achieve this, we add SYNC to it, through the mechanism of
SHIL.

	A nonlinear self-sustaining oscillator under perturbation can be described
	mathematically as a set of Differential Algebraic Equations (DAEs):
	\begin{equation}\label{eq:DAE}
		\frac{d}{dt} \vec q(\vec x) + \vec f(\vec x)  + \vec b(t) = \vec 0
	\end{equation}
	where $\vec x \in \mathbf{R}^n$ are the unknowns in the system, 
	$\vec b(t)$ is a small time-varying input.
	The oscillator's response can be approximated well as
	\begin{equation}\label{eq:xt}
		\vec x(t) = \vec x_s(t + \alpha(t))
	\end{equation}
	where $x_s(t)$ is the oscillator's steady state response without perturbation
    ($\vec b(t) \equiv \vec 0$);
	$\alpha(t)$ is the phase shift caused by the external input and is governed
	by the following differential equation:
	\begin{equation}\label{eq:PPV}
		\frac{d}{dt} \alpha(t) = \vec v^T(t + \alpha(t)) \cdot \vec b(t)
	\end{equation}
	where the vector $\vec v(t)$ is known as the Perturbation Projection Vector
	(PPV) \cite{DeMeRoTCAS2000} of the oscillator.
	Assume the oscillator's natural frequency is $f_0 = 1/T_0$.
	% its steady state response without perturbation ($\vec b(t)
	% \equiv \vec 0$) is a $T_0$-periodic function $x_s(t)$,
	% its response under perturbation can be approximated well as
	Then $\vec v(t)$ is a $T_0$-periodic vector that can be extracted
	numerically from the DAEs of the oscillator without knowing any information
	about the input $\vec b(t)$.
	Put in other words, it is a property intrinsic to the oscillator that 
	captures its phase response to small external inputs.

	PPV can be used to model and predict injection locking effectively
	\cite{LaRoMTT2004}.
	Based on it people have developed a simplified approximation of (\ref{eq:PPV})
	known as the Generalized Adler's Equation (GAE) \cite{BhRoASPDAC2009}.
	It governs the dynamics of the oscillator's phase with specific periodic
	inputs $\vec b(t)$ and its equilibrium states provide good approximations to
	injection-locked solutions of (\ref{eq:PPV}).
	GAE has the following form:
	\begin{equation}\label{eq:GAE}
		\frac{d\Delta \phi(t)}{dt} = -(f_1-f_0) + f_0 \cdot g(\Delta \phi(t))
	\end{equation}
	where $\Delta \phi(t) = f_0t+f_0\alpha(t)-f_1t$ is phase difference between
	the oscillator and the perturbation signal; $f_1$ is the fundamental
	frequency of periodic input $\vec b(t)$ and $f_1 \approx f_0$; function $g$
	is derived from (\ref{eq:PPV}) and can be evaluated numerically based on
	the formulation in \cite{BhRoASPDAC2009}.

	When injection locking happens, the phase difference $\Delta \phi(t)$
	between oscillator and injected signal becomes constant, i.e.
	\begin{equation}\label{eq:GAElock}
		\frac{f_1-f_0}{f_0} = g(\Delta \phi^*)
	\end{equation}

	By plotting the LHS and RHS of (\ref{eq:GAElock}) and looking for
	intersections, designers can predict whether IL or SHIL will happen
	given a design \cite{NeRoDATE2012SHIL} without running long and expensive
	transient simulations.

\begin{equation}
	\frac{d}{dt} \phi_i = \sum_j J_{ij} \cdot \sin(\phi_i - \phi_j),
\end{equation}

\begin{equation}
	\frac{d}{dt} \phi_i = \sum_j J_{ij} \cdot \sin(\phi_i - \phi_j),
\end{equation}
where $\phi_i$ is the ith entry of $\vec \phi$.


\begin{equation}
	E = \sum_{i, j} J_{ij} \cdot \cos(\phi_i - \phi_j).
\end{equation}

\begin{align}
	\frac{dE}{dt} &= \sum_{i} \left[ \frac{dE}{d\phi_i} \cdot
                     \frac{d\phi_i}{dt} \right] \\
				  &= \sum_{i} \left[ - \left( \sum_{j} J_{ij} \cdot
					 \sin(\phi_i - \phi_j)\right) \cdot \frac{d\phi_i}{dt}
                     \right] \\
	              &= - \left|\left|\frac{d\vec \phi}{dt}\right|\right|_2^2 \leq 0.
\end{align}

\begin{equation}
	\frac{d}{dt} \phi_i = \sum_j \left[J_{ij} \cdot \sin(\phi_i - \phi_j)
						+ K \cdot \sin\left(2\cdot (\phi_i -
                          \phi_j)\right)\right].
\end{equation}

\begin{align}
	E & = \sum_{i, j} \left[ J_{ij} \cdot \cos(\phi_i - \phi_j)
	  + \frac{K}{2} \cdot \cos\left(2\cdot (\phi_i - \phi_j)\right) \right] \\
	  & = \sum_{i, j} J_{ij} \cdot \cos(\phi_i - \phi_j)
	  + \frac{1}{2}n\cdot m\cdot K.
\end{align}


\begin{equation}
	\frac{d}{dt} \phi_i = \omega_i
	                    + \sum_j \left[J_{ij} \cdot \sin(\phi_i - \phi_j)
						+ K \cdot \sin\left(2\cdot (\phi_i -
                          \phi_j)\right)\right].
\end{equation}

\begin{equation}
	E = \sum_{i} \omega_{i} \cdot \phi_i
	    + \sum_{i, j} J_{ij} \cdot \cos(\phi_i - \phi_j)
	    + \frac{1}{2}n\cdot m\cdot K.
\end{equation}



==> newcommands-colours.tex <==
% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings


==> newcommands-eg-ie-etc.tex <==
% eg, ie, etc, wrt, viz newcommands
\newcommand{\eg}{{\it e.g.\/}}
\newcommand{\ie}{{\it i.e.\/}}
\newcommand{\wrt}{{\it wrt}}
\newcommand{\viz}{{\it viz.\/}}
\newcommand{\vs}{{\it vs.\/}}
\newcommand{\aka}{{\it aka\/}}
\newcommand{\apriori}{{\it a priori}}
\newcommand{\etc}{\textit{etc.}}                                                
% etc defined so that there is only a single period after it if it is followed 
% by a period
% see: http://en.wikibooks.org/wiki/TeX/def                                      
% see: http://www.tug.org/pipermail/texhax/2004-July/002449.html                 
% see: http://en.wikibooks.org/wiki/TeX/if                                       
%\ifx \etc \undefined                                                             
%  %\def\myarg{#1}                                                                
%  %\def\myfullstop{.}                                                            
%  %\def\etc{#1}{\textit{etc} arg is ``\myarg'' \ifx\myarg\myfullstop\then.\else.#1\fi\/}
%  \def\etc#1{\textit{etc}\if#1..\else.#1\fi}                                     
%\fi                                                                              
%                        


==> newcommands-for-bibtex.tex <==
\newcommand{\BP}{({\textbf{Best Paper}})} % used in bibliography
\newcommand{\BPnom}{({\textbf{Best Paper Nomination}})} % used in bibliography
\newcommand{\IP}{({\textbf{Invited}})} % used in bibliography
\newcommand{\presenter}[1]{#1} % used in bibliography
\newcommand{\putDOI}[1]{#1}
%\newcommand{\putDOI}[1]{}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}


==> newcommands-highlight-ignore.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands for ignoring, commenting, annotating, highlighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\newcommand{\jques}[1]{{\color{blue}#1?}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{\uline{#1}}}}
\ignore{
    \newcommand{\jnote}[1]{% using fixme
    	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
    	\renewcommand{\fixmelogo}{}%
    	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
                {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
                \textit{\color{mydarkgreen}#1}}}}%
    }
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END newcommands for ignoring, commenting, ....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> newcommands-labels-refs.tex <==
% label and ref newcommands
% now mostly deprecated (but redefined and kept for backward compatibility) - move to \cref from the cleveref package
\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\Crefname{equation}{}{}

%DONE: xyzref{} should be able to handle multiple arguments so that you can
%reference multiple figures/equations at the same time -AG
%Now fixed with some package/command CREF.
\newcommand{\corrlabel}[1]{\label{corr:#1}}
\newcommand{\corrref}[1]{Corollary \ref{corr:#1}}
\newcommand{\assref}[1]{Assumption \ref{ass:#1}}
\newcommand{\asslabel}[1]{\label{ass:#1}}
%\newcommand{\eqnref}[1]{(\ref{eq:#1})}
%\newcommand{\eqnlabel}[1]{\label{eq:#1}}
\newcommand{\eqnlabel}[1]{\label{#1}}
\newcommand{\eqnref}[1]{\cref{#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figlabel}[1]{\label{#1}}
\newcommand{\figref}[1]{\cref{#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\exampleref}[1]{Example~\ref{ex:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\thlabel}[1]{\label{th:#1}}
\newcommand{\thref}[1]{Theorem~\ref{th:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem \ref{thm:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma \ref{lem:#1}}
\newcommand{\examplelabel}[1]{\label{ex:#1}}
\newcommand{\labexample}[1]{\label{example:#1}}
\newcommand{\refexample}[1]{Example{ }\ref{example:#1}}
\newcommand{\httpref}[1]{}
\let\el=\eqnlabel
\let\er=\eqnref


==> newcommands-math.tex <==
\newcommand{\ddt}[2]{{\frac{d}{d #2}\left. #1 \right.}}
\newcommand{\ddx}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\Ddx}[2]{{\frac{D}{d{#2}}\left[ #1 \right]}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\deq}{=}
\newcommand{\I}{I\left[\right]}
\newcommand{\ELL}[1]{L\left[#1\right]}
\newcommand{\w}{\omega}
\newcommand{\calD}{{\cal D}}
\renewcommand{\jmath}{j}
\newcommand{\Pinvt}{{P(t)}^{-1}}
\newcommand{\halmos}{\hskip\textwidth minus\textwidth \rule{6pt}{6pt}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calAT}{{\cal A}^T}
\newcommand{\calL}{{\cal L}}
\newcommand{\calLadj}{\calL^\dagger}
\newcommand{\calR}{{\cal R}}
\newcommand{\Reals}{\Bbb{R}}
\newcommand{\Real}{\Bbb{R}}
\newcommand{\Safe}{\ensuremath{{\bf S}}}
\newcommand{\Pade}{{Pad\'e}}
\newcommand{\Complexes}{\Bbb{C}}
\newcommand{\HvecqLanc}{\Hvec^{(L)}_q}
\newcommand{\HvecqArn}{\Hvec^{(A)}_q}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\calDT}{{\cal D}^T}
\newcommand{\calCtil}{\tilde{\cal C}}
\newcommand{\calJtil}{\tilde{\cal J}}
\newcommand{\calDtil}{\tilde{\cal D}}
\newcommand{\JstarDphi}{J_{\Delta \phi}^*}
\newcommand{\Jstarphi}{J_{\phi}^*}
\newcommand{\vecbphi}{\vec b_{\phi}}
\newcommand{\vecbext}{\vec b_{\text{ext}}}
\newcommand{\phistarIdeal}{\phi_{\text{ideal}}^*}
\newcommand{\apdx}[1]{\appref{#1}} 
\newcommand{\delbydel}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\delbydeln}[3]{\ensuremath{\frac{\partial^{{#1}}
{#2}}{\partial{#3}^{{#1}}}}}
\newcommand{\delbydelat}[3]{\ensuremath{\left. \frac{\partial
{#1}}{\partial {#2}} \right|_{{#3}}}}
\newcommand{\dee}{\ensuremath{\mathrm{d}}}
\newcommand{\dbyd}[2]{\ensuremath{\frac{\mathrm{d} {#1}}{\mathrm{d}
{#2}}}}
\newcommand{\dbydn}[3]{\ensuremath{\frac{\mathrm{d}^{{#1}}{#2}}
{\mathrm{d}{#3}^{{#1}}}}}
\newcommand {\dist}[1] {{{\rm dist}\left({#1}\right)}}
\def\Matrix#1{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\textdiag}{{\text{diag}}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\del}{\nabla}
\newcommand{\Rxx}{R_{\vec x \vec x}}
\newcommand{\Sxx}{S_{\vec x \vec x}}
\newcommand{\Snn}{S_{\vec n \vec n}}
\newcommand{\vecphi}{\vec \phi}
\newcommand{\Dphi}{\Delta \phi}
\newcommand{\vecDphi}{\vv{\Delta \phi}}
\newcommand{\dphi}{\delta \phi}
\newcommand{\vecdphi}{\vv{\delta \phi}}
\newcommand{\ah}{\alpha_g} % g for group
%\newcommand{\tDagger}{{\tilde t}}
\newcommand{\tDagger}{{t^{\!\dagger}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\texthyphen}{\text{--}}

%The substack command can be used to produce a multi-line subscripts or superscripts:
%\sum_{\substack{0\le i\le m\\ 0<j<n}} P(i,j) produces a two-line subscript underneath the sum.
%A slightly more general form is the subarray environment which allows you to specify that each line should be left-aligned instead of centered, as here:
% \sum_{\begin{subarray}{l} i\in\Lambda\\ 0<j<n \end{subarray}} P(i,j) 

%\newcommand{\be}[1]{\begin{equation}\eqnlabel{#1}} % now moved to cleveref
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\def\ee{\end{equation}}


==> newcommands-squeeze-spaces.tex <==
%%% tweaklist renewcommands
\newcommand{\modifiedListParamters}{
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.1em}
  \setlength{\partopsep}{0em}
  \setlength{\parsep}{0em}
  \setlength{\leftmargin}{1.1em}
  \setlength{\itemindent}{0.0em}
}
\renewcommand{\enumhook}{
  \modifiedListParamters
  \setlength{\itemindent}{0.2em}
}
\renewcommand{\itemhook}{
  \modifiedListParamters
}
\renewcommand{\descripthook}{
  \modifiedListParamters
  \setlength{\itemindent}{-1.0em}
}
%%% end tweaklist renewcommands

\ignore{not usually needed, but the definitions have useful info
		Space saving List environment for enumerations.

	\newcounter{myctr}
	\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
   		{\usecounter{myctr}
   		%\setlength{\topsep}{1mm}\setlength{\itemsep}{0.5mm}
   		\setlength{\topsep}{0.3mm}
   		\setlength{\itemsep}{0mm}
   		\setlength{\parsep}{0.3mm}
   		\setlength{\itemindent}{0mm}
   		\setlength{\partopsep}{0mm}
   		\setlength{\labelwidth}{15mm}
   		\setlength{\leftmargin}{4mm}
   		}
	}{\end{list}}

	\newenvironment{myitemize}{\begin{list}{$\bullet$}
	  \ignore{\setlength{\topsep}{0.8mm}\setlength{\itemsep}{0.25mm}}
	  {\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
	  \setlength{\parsep}{0.1mm}
	  \setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
	  \setlength{\labelwidth}{15mm}
	  \setlength{\leftmargin}{4mm}}
	}{\end{list}}
}

%%%% titlesec: squeezing whitespace between section headings
	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
                                           % space above; {*0.5} is space below
	\titlespacing{\subsection}{0pt}{*0.1}{*0}
	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%% end titlesec

%%%% squeezing whitespace in and around figures
    \floatsep=0em % space left between floats.
    \textfloatsep=0em % space between last top float or first bottom float and the text.
    \intextsep=0em % space left on top and bottom of an in-text float.
    %\dbltextfloatsep is \textfloatsep for 2 column output.
    %\dblfloatsep is \floatsep for 2 column output.
    \abovecaptionskip=0em % space above caption
    \belowcaptionskip=0.3em % space below caption
%%%% END squeezing whitespace in and around figures

\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

%\newcommand{\mycaption}[1]{\caption{\small #1}}
\newcommand{\mycaption}[1]{\caption{\tiny #1}}

% for captions spacing
\captionsetup[table]{font={scriptsize},format=hang,indention=0em}     %% change 1.2 as you like
\captionsetup[figure]{font={scriptsize},format=hang,indention=0em}    %% change as you like
 %% or
 %% \captionsetup{font={stretch=1.2}}  %% this affects both figure and table

% replace Figure x in captions by Fig. x
%\renewcommand{\figurename}{Fig.} % doesn't work.
%but \usepackage[figurename=Fig.]{caption} in packages-headers.tex does work.


%\renewcommand{\baselinestretch}{1.5}
%\setstretch{1.5}

%\def\baselinestretch{0.8593}\large\normalsize - this form works locally?
%\renewcommand{\baselinestretch}{0.94} - this form works only in the preamble
%\renewcommand{\baselinestretch}{0.90}
%\renewcommand{\baselinestretch}{0.5}
%\linespread{0.5} % 0.5 -> 7 lines per inch; 0.9 -> a bit more than 6 lines 
%                 % per vertical inch
% \linespread{0.99}

% baselinestretch fixes for squeezing. See also linespread
%\def\ssp{\def\baselinestretch{0.95645}\large\normalsize} % "single space"
%\def\ssp{\def\baselinestretch{0.905}\large\normalsize} % "single space"
\def\ssp{\def\baselinestretch{0.9}\large\normalsize} % "single space"
\def\dsp{\def\baselinestretch{1.35}\large\normalsize} % "double space"
\ssp

% indent paragraphs less (saves space)
\parindent 	1em
% do not indent paragraphs (saves more space)
\parindent 	0em
% adjust space between paragraphs (0em can obscure paragraph breaks)
\parskip 0.3em


==> newcommands-thm-env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EndProof{\hfill \quad \vrule width 1ex height 1ex depth 0pt  }
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{illustration}{Illustration}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newenvironment{sketch}{\noindent{\bf Sketch of Proof}:}{\halmos}
\newenvironment{conjecture}{\noindent{\bf Conjecture}: \em}{}
\newcommand{\numberedtheorem}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thetheorem
		\renewcommand{\thetheorem}{#1}
	}
	\begin{theorem}
	\ifthen{\not\equal{#2}{}}{
		\thmlabel{#2}
	}
	#3
	\end{theorem}
	\ifthen{\not\equal{#1}{}}{
		\let\thetheorem=\oof
		\addtocounter{theorem}{-1}
	}
}
\newcommand{\numberedlemma}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thelemma
		\renewcommand{\thelemma}{#1}
	}
	\begin{lemma}
	\ifthen{\not\equal{#2}{}}{
		\lemlabel{#2}
	}
	#3
	\end{lemma}
	\ifthen{\not\equal{#1}{}}{
		\let\thelemma=\oof
		\addtocounter{lemma}{-1}
	}
}


==> packages-headers.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
%\RequirePackage[usenames]{pstcol} 
\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsthm,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage{hyperref} 
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{MyDarkRed}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}


\input newcommands-colours
\input newcommands-highlight-ignore
\input newcommands-eg-ie-etc
\input newcommands-labels-refs
\input newcommands-math
\input newcommands-thm-env
\input newcommands-for-bibtex
\input newcommands-squeeze-spaces

